Predictability of Performance in Communication Networks Under Markovian Dynamics

With the emergence of time-critical applications in modern communication networks, there is a growing demand for proactive network adaptation and quality of service (QoS) prediction. However, a fundamental question remains largely unexplored: how can we quantify and achieve more predictable communication systems in terms of performance? To address this gap, this paper introduces a theoretical framework for defining and analyzing predictability in communication systems, with a focus on the impact of observations for performance forecasting. We establish a mathematical definition of predictability based on the total variation distance between forecast and marginal performance distributions. A system is deemed unpredictable when the forecast distribution, providing the most comprehensive characterization of future states using all accessible information, is indistinguishable from the marginal distribution, which depicts the system's behavior without any observational input. This framework is applied to multi-hop systems under Markovian conditions, with a detailed analysis of Geo/Geo/1 queuing models in both single-hop and multi-hop scenarios. We derive exact and approximate expressions for predictability in these systems, as well as upper bounds based on spectral analysis of the underlying Markov chains. Our results have implications for the design of efficient monitoring and prediction mechanisms in future communication networks aiming to provide deterministic services.

==> reviewerscomments.tex <==

Dear Mr. Mostafavi:

The review of your paper

VT-2024-04811: Predictability of Performance in Communication Networks Under Markovian Dynamics

has been completed.  Below please find comments from the reviewers.

Based on the reviewers' comments, publication of the paper in its present form is not recommended.  It is recommended that you resubmit your manuscript, WITHIN TWO MONTHS from the date of this email, as revised in accordance with the comments. If you fail to do so, your paper will be considered withdrawn from the review process.

In particular, the paper needs to be positioned better to be aligned with the theme of TVT. Additionally, the considered performance measures need to be sufficiently justified. The detailed comments and concerns of the reviewers need to be carefully addressed. 


Please note that this recommendation of resubmission should not be treated as an implication of eventual acceptance of your paper. It only refers to a deferral of the editorial decision to see whether the reviewers' comments could be addressed. In the event that your revision is accepted, the  manuscript must be in a format that is in accordance with IEEE final submission requirements. For detailed final submission requirements, kindly refer to the information for IEEE Authors guidelines  contained on the website http:/www.ieee.org/pubs/authors.html.

PLEASE READ:
If you originally submitted via the IEEE Author Portal, please upload your files here: https://ieee.atyponrex.com/journal/tvt-ieee

If you originally submitted via ScholarOne Manuscripts, please upload your files here: https://mc.manuscriptcentral.com/tvt-ieee


Please note that your manuscript (including main body, figures, tables, references) should be in double-columned with fonts no smaller than 10pt in the final IEEE typesetting with maximum page length 16 pages for regular papers.

Additionally, you MUST submit a response file alongside you manuscript that details the changes you have made and addresses the issues raised by the reviewers. REVISION WITHOUT THIS FILE WILL BE REJECTED. 

The revised manuscript should follow our submission policy. The complete revised manuscript (including main body, figures, tables, references, and appendix) of a Regular Paper should be in general limited to 35 pages. If the revised paper does not comply our submission policy, it may be considered withdrawn without the review process.

As the system keeps all the files from your earlier submission(s) for this paper, please remember to delete any files which are not part of this new revised submission.


Sincerely,

Swades De
Editor, IEEE Transactions on Vehicular Technology


==============================================
Reviews for VT-2024-04811

*Please note that there may be attached files that contain additional
comments from the reviewers. To see these files, please log on to
your "Author Center" at the Manuscript Central web site
(https://mc.manuscriptcentral.com/tvt-ieee) and select this paper to
see and download the files.
==============================================

Reviewer: 1

ADDITIONAL COMMENTS TO THE AUTHOR:
The paper presents a new definition of network predictability performance in Markovian conditions. The framework is applied to Geo/Geo/1 queuing models in single hop and multi-hop context. The following are the comments with respect to the paper, which should be incorporated/clarified as appropriate.

1. In related works section, the authors describe autocorrelation, entropy, and information theoretic measures existing in literature to measure predictability. Please comment on the need for a new metric as presented in this paper and the short comings of the aforementioned ones.

2. The authors should incorporate some cross entropy based results since they are measuring the "distance" between the conditional and marginal distributions in the new proposed metric. This will help in getting an idea of the efficacy of the new metric as compared to cross entropy which has been widely studied.

3. The authors may motivate the paper more from a vehicular networks perspective considering the scope of the transaction.

4. The write up of System model should be simplified. While it understandable, it may be tough for beginners. For instance, Fig. 1 and Fig. 2 can be explained and motivated together in the beginning of Section III. The variables $Z_n$ and $X_n$ should be first well explained, following which the math equations may start. The queuing model can also be explained before starting the equations. Better structuring of Sec. III will help to improve the quality of paper. The section can also be structured in multiple subsections to bring more clarity.

5. The authors should justify the various assumptions used in Sec. III, e.g., stationary distributions and independence.

6. A table of parameters and their meanings will be very helpful.

7. The assumption of stationarity should be clearly mentioned in the proposed definition of predictability.

8. The authors have simulation results with $\rho$ < 1 in all cases. It is suggested to show results for $\rho$ =1 and $\rho$ > 1. These cases are crucial for testing the framework in more practical scenarios.

9. The authors should also vary K and L and showcase some results.

10. It seems that the number of hops has been fixed. Visualizing network performance with respect to varying number of hops might be of interest.

11. What is the "QoS" value or the latency budget value considered in simulations. It is not very clear.

Reviewer: 2

ADDITIONAL COMMENTS TO THE AUTHOR:
This paper introduces a theoretical framework for defining and analyzing predictability in communication systems. There are several concerns as follows.
1.The logic of introduction is a bit confusing. The relationship among the paragraphs in the introduction should be improved.
2.Both the past tense and present tense are adopted by authors to introduce the related works, which should be improved. Some references are outdated, and should be updated by latest related works.
3.Why authors adopt three different observability defects in the model? More details and explanations should be provided, and how these three cases are applicable?
4.In my point of view, the multi-hop communication system model in figure 1 is a bit ideal. The multi-hop communication structure could be more general.
5.There are many writing issues in the manuscript, such as “first, delayed observations, which is particularly crucial when a network of remote nodes is involved in the packet route.” In page 3, and “Total Variation distance (TV)” in page 4 should be revised as “Total Variation (TV) distance”.
6.Authors adopt many assumptions in the system model, which require details explanations.
7.According to proposition 1, the authors derived the predictability of the sojourn time of a Geo/Geo/1/K queue with a very large K. In other values of K, how the predictability of the sojourn time of a Geo/Geo/1/K queue could be obtained?
8.The impacts of imperfect observations on the network performance of multi-hop systems should be provided in numerical evaluations.

Reviewer: 3

ADDITIONAL COMMENTS TO THE AUTHOR:
This manuscript introduces a theoretical analysis of predictability in communication systems. The mathematical framework is based on the total variation distance between forecast and marginal performance distributions. The authors have analyzed G/G/1 queuing models with single-hop and multi-hop scenarios. They also derived exact and upper bound expressions for predictability. Furthermore, the paper is well written with appropriate sections and titles.

1. The authors should compare this work with more predictability-related works on communication systems. They have cited only two related works [30,31] on this area; however, they seem to be almost a decade old. I suggest the authors include more recent literature if possible and benchmark the results.

2. The authors consider two Markovian assumptions to analyze the performance in communication systems: performance at time slot n depends only on the observations at n and observations at n depends only on the observations at time n-1. It is not clear which use cases or performance measures satisfy this behavior. I suggest the authors to provide more examples or application measures to make it clear.

3. The trends of the curves in the numerical plots have not been explained well. For example, the predictability decreases as lead time decreases; and the decrease is exponential/linear depending on the other parameters. I see the authors have explained the changes in the decrease for Figs. 9 and 10. However, it would be more clear to explain the trends in the initial figures first and then explain the changes in the decrease.

4. The authors mention in the explanation for Fig.6 that the spectral-based upper bound in Theorem 2 is not accurate for the large queue sizes. However, the reasoning for this gap is not addressed at all. I suggest the authors to properly give the reasons or the limitations for the usage of Theorem 2.

5. I see few presentation conflicts in the paper.

a. Some of the mathematical notations are not defined before using them in the paper. For example, state space X and its size K were not defined properly.
b. Few notations have been reused: $\lambda$ has been used for eigenvalues and arrival rates.
c. I suggest the authors to include a subsection for notations before system model and define all the notations beforehand. For example: probability, conditional probability, total variation distance and cardinality of a set can be predefined.
d. Punctuations are missing in the equations in appendix B and in equation 41.
